Hawkes Process Multi-armed Bandits for Disaster Search and Rescue

We propose a novel framework for integrating Hawkes processes with multi-armed bandit algorithms to solve spatio-temporal event forecasting and detection problems when data may be undersampled or spatially biased. In particular, we introduce an upper confidence bound algorithm using Bayesian spatial Hawkes process estimation for balancing the tradeoff between exploiting geographic regions where data has been collected and exploring geographic regions where data is unobserved. We first validate our model using simulated data and then apply it to the problem of disaster search and rescue using calls for service data from hurricane Harvey in 2017. Our model outperforms the state of the art baseline spatial MAB algorithms in terms of cumulative reward and several other ranking evaluation metrics.

==> algo_sim.tex <==
\begin{algorithm}[ht]
    \caption{Spatial-temporal Events Simulation}
    \label{alg:sim}
    \begin{algorithmic}[1]
        % 
        \Procedure{SynSim}{$T, \eta, \phi, \omega, \sigma$}
                \State Initial $\Event \in \{\}$, $j$ = $1$, 
                $n \leftarrow \mathcal{P}(\eta T)$ \label{algo:line:Imt}
                %
                \For{$i=1$ to $n$}
                    \State $\hat{t_i} \leftarrow  \mathcal{U}(0, T)$ \label{algo:line:ImtT}
                    \State $\hat{x_i}, \hat{y_i} \leftarrow  \mathcal{U}(0, 1)$\label{algo:line:ImtS}
                    \State $\Event = \Event \bigcup \{\Event_{i}: (\hat{t_i}, \hat{x_i}, \hat{y_i})\}$
                \EndFor
 
                \While { $|\Event|$ $>=$ j}
                    \State $K \leftarrow \mathcal{P}( \phi )$ \label{algo:line:off}
                    \For{$k=1$ to $K$}
                        \State $\Delta t \leftarrow \mathcal{E}( \omega )$ \label{algo:line:offT}
                        \State $\Delta x, \Delta y \leftarrow \mathcal{N}(0, \sigma)$\label{algo:line:offP}
                        \If{$\hat{t_j}+\Delta t \leq T$ \textbf{and} $\hat{x_j}+\Delta x, \hat{y_j}+\Delta y \leq 1$ }
                            \State $\Event = \Event \bigcup \{\Event_{n + 1}: (\hat{t_j}+\Delta t, \hat{x_j}+\Delta x, \hat{y_j}+\Delta y)\}$
                        \EndIf
                        %\State $n = n + 1$
                    \EndFor
                    \State $j$ = $j+1$
                \EndWhile
        %
        \EndProcedure
    \end{algorithmic}
\end{algorithm}



==> figure/Num_eachVisit/Num_eachVisit.tex <==
                                     % size w, h
        \begin{gnuplot}[ terminal=pdf,terminaloptions={size 3.4, 2.7}]

            # point type :https://blog.twei7.com/wp-content/uploads/2016/02/gnuplot-line-and-point-types-bw.png
            
            reset
            unset key
            
            bm = 0.15
            lm = 0.18
            rm = 0.95
            gap = 0.04
            size = 0.7
            kk = 0.8 # relative height of bottom plot
            y1 = 0.0; y2 = 15.0; y3 = 180.0; y4 = 220.0

            set xtics font ", 10"
            set ytics font ", 10"
            set xlabel "Time (seconds)"
            set ylabel "Number of events"

            # http://materials.ucsd.edu/doc/ps_guide.pdf
            # set delimeters that you use for your data
            set datafile separator ","
            
            
            set multiplot
            
            set label '\~' at   -5, 272 font ", 20"
            set label '\~' at   -5, 290 font ", 20"
           
            set label '\~' at   195, 272 font ", 20"
            set label '\~' at   195, 290 font ", 20"
            set label '×10^5' at  185, -50 font ", 10"
           # set label "Number of events"  at -20, 120 font ", 10" rotate by 90
            
            
            set border 1+2+8
            set xtics nomirror
            set ytics nomirror
            
            set lmargin at screen lm
            set rmargin at screen rm
            set bmargin at screen bm
            set tmargin at screen bm + size * kk
            
            set xrange [  0:200]
            set yrange [  0:270]
            set xtics ("0" 0, "9" 50, "18" 100, "27" 150, "36" 200)
            
            set ytics (50, 100, 150, 200, 250)
            set boxwidth 0.60
            set style fill solid
	        plot "./figure/Num_eachVisit/num_eachVisit.txt" using 1:2 with boxes linecolor 'blue'
	        
          
	        unset xtics
            unset xlabel
            unset ylabel
            set border 2+4+8
            set bmargin at screen bm + size * kk + gap
            set tmargin at screen bm + size + gap
            set xrange [  0:200]
            set yrange [400:415]
            set ytics (410, 420 ,430)
            plot "./figure/Num_eachVisit/num_eachVisit.txt" using 1:2 with boxes linecolor 'blue'
            # 
            
 
            
        \end{gnuplot}



==> table/Overall_Performance.tex <==
\begin{table*}[ht]
  \begin{minipage}[t]{0.49\linewidth}
   %  \vspace{-14pt}
  \centering
  \caption{Best Performance on $\mathcal{D}_{\text{Hry}}$ }
  \label{table:permWAll}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{2pt}} 
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{0pt}}
        }
        \toprule 
        &&&&&&&&\\[-12.5pt]
         Model & $\overline{\text{reward}}$ & NDCG & mRHR & Rec & Prec & F1 & $\overline{\text{Prec}}$ & $\overline{\text{AgPrec}}$ \\
        \midrule
&&&&&&&&\\[-12.5pt]

\EpiGreedy  & 0.1766          & 0.2224            & 0.1345            & 0.1758	        & 0.2152	        & 0.1928	        & 0.2719            & 0.3285            \\
\UCBone     & 0.1897          & 0.2917            & 0.1669            & 0.2032	        & 0.2547	        & 0.2233	        & 0.3106            & 0.3943            \\
\UCBHp      & 0.2122          & 0.3198            & 0.1880            & 0.2286	        & 0.2649	        & 0.2367	        & 0.3284            & 0.4460            \\
\UCBoneHpSp & 0.2181          & 0.3502            & 0.2016            & 0.2404	        & 0.2679	        & 0.2491	        & 0.3413            & 0.4613            \\
\GPUCB      & 0.2473          & 0.3440            & 0.1963            & 0.2489	        & 0.2956	        & 0.2697	        & 0.3728            & 0.4487            \\
\model      & \textbf{0.2546} & \textbf{0.3584}   & \textbf{0.2087}   & \textbf{0.2633}	& \textbf{0.3074}	& \textbf{0.2834}   & \textbf{0.3920}   & \textbf{0.4661}   \\ [-1.5pt]


        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
        \item
           The best performance is marked in \textbf{bold}. \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  \end{small}
  \end{minipage}\hfill
%
  \begin{minipage}[t]{0.49\linewidth}
     \vspace{-1pt}
  \centering
  \caption{Performance on $\mathcal{D}_{\text{Hry}}$ Corresponding to Best $\overline{\text{reward}}$}
  \label{table:permWAll}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{2pt}} 
          @{\hspace{2pt}}r|@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{0pt}}
        }
        \toprule
        &&&&&&&&\\[-12.5pt]
Model   & $\overline{\text{reward}}$      
         & NDCG & mRHR & Rec & Prec & F1 & $\overline{\text{Prec}}$ & $\overline{\text{AgPrec}}$ \\
        \midrule
&&&&&&&&\\[-12.5pt]

\EpiGreedy   & 0.1766          & 0.2125            & 0.1254            & 0.1602            & 0.2034            & 0.1790            & 0.2520            & 0.2862 \\
\UCBone      & 0.1897          & 0.2714            & 0.1581            & 0.1991            & 0.2547            & 0.2233            & 0.3106            & 0.3460 \\
\UCBHp       & 0.2122          & 0.3042            & 0.1697            & 0.2205            & 0.2392            & 0.2295            & 0.3140            & 0.3956 \\
\UCBoneHpSp  & 0.2181          & 0.3349            & 0.1850            & 0.2308            & 0.2523            & 0.2409            & 0.3288            & \textbf{0.4323} \\
\GPUCB       & 0.2473          & \textbf{0.3366}   & \textbf{0.1912}   & \textbf{0.2489}   & \textbf{0.2956}   & \textbf{0.2697}   & \textbf{0.3728}   & 0.4125 \\
\model       & \textbf{0.2546} & 0.3070            & 0.1717            & 0.2238            & 0.2776            & 0.2475            & 0.3455            & 0.3819 \\[-1.5pt]

        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
        \item
           temp \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  \end{small}
  \end{minipage}\hfill

\end{table*}


==> table/Overall_Performance_NavyData.tex <==
\begin{table}[ht]
%  \vspace{-14pt}
  \centering
  \caption{Overall Performance NavyData (838 events)}
  \label{table:permWAll}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}[]{
          @{\hspace{0pt}}l@{\hspace{4pt}} 
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{10pt}}
        }
        \toprule
        
        %  the optimal reward: 3701
                Model           & \# Events         & Recall & NDCG & $\text{OptRecall}_{\text{avg}}$  \\
        \midrule
            \EpiGreedy          & 285.77            & 0.3410 & 0.4524 & 0.3391 \\
            \LinUCB             & 125.00            & 0.1492 & 0.2328 & 0.1664 \\
%            \LinUCBSim          & 526.73        
            \GPOnline           &  84.58            & 0.1009 & 0.1392 & 0.1021 \\
            \UCBone             & 540.48            & 0.6450 & 0.6601 & 0.5918 \\ \hline 
            %\UCBoneHawkes       & 542.66            & 0.6476 & 0.6605 & 0.5957 \\
            %\UCBoneHawkesSim    & 569.58            & 0.6797 & 0.6733 & 0.6200 \\
            \UCBoneHawkesCI     & \textbf{-}   & \textbf{-} & \textbf{-} & \textbf{-} \\
        %
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \setlength\labelsep{0pt}
        \begin{scriptsize}
        \item
           There are $1,971$ records in total and only $838$ have address and correct time stamp.  \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  \end{small}
% \vspace{-18pt}
\end{table}


==> table/ParaStudy_Zeta.tex <==
\begin{table}[h]
  \caption{Definitions and Notations}
  \label{tbl:Notation}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
          @{\hspace{2pt}}r@{\hspace{4pt}} 
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
          @{\hspace{4pt}}r@{\hspace{4pt}}
        }
            \toprule
                \diagbox[innerwidth=8pt, height=0.9\baselineskip, innerrightsep=0pt, innerleftsep=2pt]
               {$\zeta_{\text{Hp}}$}{$\zeta_{\text{Sp}}$}
                %{ \multicolumn{1}{r}{$\gamma$} }{ \multicolumn{1}{l}{$\sigma$} } 
                & 0.01 & 0.1 & 1 & 10 & 100 \\
            \midrule
         0.0001  & 0.1737 & 0.2213 & \textbf{0.2546} & 0.2417 & 0.2105 \\
         0.01    & 0.1737 & 0.2213 & \textbf{0.2546} & 0.2417 & 0.2146 \\
         0.1     & 0.1737 & 0.2259 & 0.2503 & 0.2107 & 0.2148 \\
         1       & 0.1772 & 0.2216 & 0.2463 & 0.2140 & 0.2157 \\
         10      & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\
            \bottomrule
      \end{tabular}
            
            
    
    
    
    
    
    
    
    
    
            
            
    
      %
      %\begin{tablenotes}
      %      \setlength\labelsep{0pt}%
      %      \begin{footnotesize}
      %              \item
      %              \par
      %      \end{footnotesize}
      %\end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}

==> table/notation.tex <==
\begin{table}[h]
  \caption{Definitions and Notations}
  \label{tbl:Notation}
  \centering
  \begin{threeparttable}
    \begin{small}
      \begin{tabular}{
        @{\hspace{2pt}}p{0.2\linewidth}@{\hspace{8pt}}
        @{\hspace{2pt}}p{0.75\linewidth}@{\hspace{5pt}}
        }
            \toprule
                notation          & description   \\
            \midrule
                %$\event$        & overdose event \\
                $V$                             & total visit in the MAB processes \\
                $W$                             & time window for each time slot \\
                $X$                             & number of partitions in longitude\\
                $Y$                             & number of partitions in latitude \\
                $N$                             & number of cells/arms to visit/pull each time \\
                $L$                             & number of sampled parameters \\
                $\arm$ and $\xa$                & cell and its corresponding feature \\
                $\boldsymbol{a}$                & selected cells for next visit \\
                $\mathrm{x}$ and $\mathrm{y}$   & grid indicator for longitude and latitude \\
                $v$                             & indicator for visits (often in superscript) \\
                $l$                             & indicator for sampled parameters \\
                $t_c$                           & timestamp for current time \\  
                $\mathcal{T}^{v}_{a}$           & set of observed timestamps for cell $\arm$ at visit $v$ \\
                %
                $\boldsymbol{\hat{\mathcal{S}}^{a}}$    & best guess on timestamps for cell $\arm$  \\
                $\boldsymbol{\widetilde{\mathcal{S}^{a}_{l}}}$      & set of simulated timestamps for $\arm$ and parameter $v$ \\
                %\boldsymbol{\widetilde{\mathcal{S}}}$      & set of observed timestamps for cell $\arm$ at visit $v$ \\
                %
                %$t$                     & timestamp \\
                %$r_a^v$                 & rewards observed from cell $\arm$ at visit $v$ \\
                %$s$                     & score generated by the algorithm \\  
                %\midrule
                %$\epsilon$                & free parameter for $\EpiGreedy$\\
                %
                %$\zeta_{\text{ucb}}$      & free parameter for $\UCBone$\\
                %
                %$\sigma_{\text{gp}}$      & free parameter for $\GPUCB$\\ 
                %$\zeta_{\text{gp}}$       & free parameter for $\GPUCB$\\ 
                %$\tau_{gp}$               & free parameter for $\GPUCB$\\
                %$\zeta_{\text{gp}}$       & free parameter for $\GPUCB$\\
                %$\mathbf{k}_\text{RBF}$   & kernel for Gaussian process\\
                %
                %$\mathcal{L}$             & likelihood functions\\
                %$\lambda$                 & intensity functions\\
                %$\mu$                     & background intensity\\
                %$\alpha$                  & infectivity factor\\
                %$\beta$                   & exponential decay rate\\
                %$\mathcal{G}(k_s, k_p)$   & gamma distribution, and its scale and shape parameters\\
                %$\mathcal{B}(m,n)$         & beta distribution and its shape parameters\\
                %
                %$\theta$                  & inferred parameters from posterior distribution\\
                %$\boldsymbol{\Theta}$     & set of inferred parameters\\
                %$\hat{\mathcal{S}_{a}}$   & best guess on simulated timestamps\\
                %$\widetilde{\mathcal{S}_{a}^{l}}$ & simulated timestamps\\
                %$\zeta_{\text{SPucb}}$           & free parameter for $\model$\\
                %$\sigma_{f}$            & free parameter for $\model$\\
                %$\gamma$                & free parameter for $\model$\\
                %\midrule
            \bottomrule
      \end{tabular}
      %
      %\begin{tablenotes}
      %      \setlength\labelsep{0pt}%
      %      \begin{footnotesize}
      %              \item
      %              \par
      %      \end{footnotesize}
      %\end{tablenotes}
    \end{small}
  \end{threeparttable}
\end{table}
